Tangi: a Tool to Create Tangible Artifacts for Sharing Insights from 360$^\circ$ Video

Designers often engage with video to gain rich, temporal insights about the context of users, collaboratively analyzing it to gather ideas, challenge assumptions, and foster empathy. To capture the full visual context of users and their situations, designers are adopting 360$^\circ$ video, providing richer, more multi-layered insights. Unfortunately, the spherical nature of 360$^\circ$ video means designers cannot create tangible video artifacts such as storyboards for collaborative analysis. To overcome this limitation, we created Tangi, a web-based tool that converts 360$^\circ$ images into tangible 360$^\circ$ video artifacts, that enable designers to embody and share their insights. Our evaluation with nine experienced designers demonstrates that the artifacts Tangi creates enable tangible interactions found in collaborative workshops and introduce two new capabilities: spatial orientation within 360$^\circ$ environments and linking specific details to the broader 360$^\circ$ context. Since Tangi is an open-source tool, designers can immediately leverage 360$^\circ$ video in collaborative workshops.

==> content/01-related-work/existing-boundary-objects.tex <==
\subsection{Examples of 360° Video Frame Artifacts}\label{bg-360-frames-hci}
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{content//images//360va/three-examples.png}
    \caption{Three examples of ways to present 360° video from~\citet{li_route_2021}. A: the standard equirectangular projection. B: the Little Planet projection suggested by~\citet{nguyen_vremiere_2017}. C: the Route Tapestries suggested by~\citet{li_route_2021}, which show the ``sides'' of a 360° video to give an overview of the timeline of a video.}
    \label{fig:existing-360-artifacts}
\end{figure}
There are a number of papers that attempt to tackle the challenge of showing a frame of 360° video (Figure~\ref{fig:existing-360-artifacts}), here we will describe several and why they do not fit the needs of VDE.
~\citet{li_route_2021} describe the concept of Route Tapestries (Figure~\ref{fig:existing-360-artifacts}), which simplifies the 360° video into two conventional videos of the sides of the street in order to provide a logical overview of a 360° video for editing. While this does reduce the distortion and provide important context, it is designed to provide an overview of the entire video and does not support connecting multiple elements of a single frame.
Other papers recommend specific projections, such as the Little Planet projection defined by~\citet{nguyen_vremiere_2017} (Figure~\ref{fig:existing-360-artifacts}), which does provide an overview of the 360° frame on a 2D plane (and thus could be made into a tangible print out), however the view is highly distorted.
~\cite{vermast_introducing_2023} explore different methods of projecting equirectangular images onto flat or 3D shapes in Virtual Reality and found spherical thumbnails resulted in a better user experiences, however, these thumbnails and the interactions with them are contained in a VR headset.
Another approach~\cite{su_pano2vid_2016,truong_tool_2019} is to use an algorithm to ``flatten'' the 360° video into a conventional video or story-board. However these techniques are based the idea that there is a single, objectively defined, area of interest -- which conflicts with the manor~\citet{meijer_sphere_2024} describe designers using multiple perspectives of a 360° video in the same moment to get insights which ``...depends on one’s interests as a designer''~\cite[p.91]{ylirisku_designing_2007}.

Largely, these methods focus on providing a simplification of 360° video aimed at digital interactions with the video (e.g., selecting a video, 360° video editing, giving an overview of the timeline of the video), and thus do not lend themselves well to the tangible, iterative nature of using frame level video artifacts during VDE workshops.


==> content/fig_desc.tex <==
Figure 1 a: a distorted view of a Paris street, it is a sphere that has been flattened into a rectangular image.
Figure 1 b: a photo of two pieces of paper, one has the flat pattern of a geodesic octahedron and the other is that pattern folded into a 3D shape. Both have the 360° image from Figure 1 a projected on it.
Figure 2 a: a subset of the image from Figure 1 a that is not distorted, but only shows a small area
Figure 2 b: the same image but with a much wider perspective - thus distorted. Call-outs show that the view includes the cyclist that took the video, the view behind them, other cyclists, as well as green spaces and weather.
Figure 3: a diagram showing the stages of the video design ethnography process. All of the stages are on one line and are (2) brief, (2,3,4) field research, (5) analysis (substages view and annotate and sense-making which are connected by an iterative process), and (6) output.
Figure 4 a: a sequence of frames from the movie Charade, showing the selection of one frame.
Figure 4 b: the frame from figure 4 a with a red arrow, speech bubble, and  sticky note to indicate additional information about the scene.
Figure 4 c: frames from diverse movies showing the concept of sneaking.
Figure 5: a design space as a 2D graph with the axes of spherical-flat and digital-tangible. On the left (digital) side there are examples of digital artifacts for 360° content, on the right there are two boxes in the lower (flat) corner showing perspective screenshots and distorted screenshots.
Figure 6: 3 examples of 360° artifacts, the first is a 3D thumbnail - a sphere that someone in VR could move around. Second the little planet projection which shows a distorted overview of the full scene. Thirdy route tapestries which show the two side views of someone traveling down a street.
Figure 7: the photo of a Paris street shown in Figure 2 a, which differing Fields of View - there is more visual information as the FOV increases, but also more distortion.
Figure 8: the design space from figure 5 with two new boxes in the tangible + spherical quadrant. One (tangi: flat) is connected to perspective screenshots. The other (tangi: sphere-ish) is connected to 3D thumbnails.
Figure 9 a: a piece of paper with a perspective crop of a larger 360° image, with the full 360° image as a map projection shown in the upper right hand corner.
Figure 9 b: the same overall 360° image projected onto a cube.
Figure 10 a: a screenshot of a web page that shows the two images from figure 9 a and b and has some text describing the two representations of 360° images
Figure 10 b: a screenshot of a web-page that shows a flat projection of the earth on the left and the same image projected on the flat pattern of a geodesic octahedron on the right.
Table 1: a simple table that lists 9 participants (P1-P9), their experience with design in years and experience with 360° video in years.
Figure 11: the cube shown in figure 9 b with some circular stickers attached to it to indicate different insights. There is a sticky note attached to the cube on a string which has text corresponding to the stickers
Figure 12 a: a hand holds up part of a piece of paper with 360° video on it, showing how an artifact might transform from flat to 3D
Figure 12 b: a single frame of 360° video that has multiple copies of the same person on it, indicating their motion around the frame
Figure 12 c: a series of paper cubes attached together, were each is a different frame of a video showing the motion of a cyclist.

==> content/old/approach.tex <==
Given that 360° video provides unique benefits for video ethnography, while at the same time complicating the creation of tangible video artifacts that support the video design ethnography process, we sought to create a Tangible 360° Video Artifact Framework to support designers to create and modify artifacts to suite their needs. To this end, we used a Research through Design (RtD) approach with the aim of creating not just a collection of artifacts, but an underlying framework to support designers in selecting, creating and modifying them. The three phases were:
\begin{enumerate}
    \item create an initial collection of tangible 360° video artifacts (Section~\ref{initial-framework}),
    \item conduct generative sessions to elicit qualities of these artifacts and create an initial framework (Section~\ref{generative-sessions}), and
    \item refine this framework by applying it to two case studies (Section~\ref{case-study}).
\end{enumerate}
% To simplify this paper, we primarily focus on the outcomes of each phase. Finally, we present the resulting Tangible 360° Video Artifact Framework in Section~\ref{framework}.

% In line with the iterative nature of RtD, each phase consisted of experimentation, prototyping, and evaluation with a group of experts and colleagues listed in Table~\ref{tab:participants}. In order to simplify this paper, Sections~\ref{initial-framework} and~\ref{generative-sessions} focus primarily on the outcomes, whereas Section~\ref{case-study} provides more details about the process. The ``final'' framework~\footnote{We believe that all design tools and techniques evolve and adapt over time, so there is no final version of the framework.} is presented in Section~\ref{framework}.

% Throughout the process we engaged with many experts and colleagues to shape the framework, those we formally engaged with during the generative sessions and the case studies are listed in Table~\ref{tab:participants}
% \begin{table}[h]
% \begin{tabular}{lll}
% Participant & Experience & Exp. with 360° video \\
% P1 & 8 years industrial design & 1 year \\
% P2 & 25+ years visual perception & 10 years \\
% P3 & 20+ years visual perception & 5 years \\
% P4 & 6 years & 1 year \\
% P5 & 10 years & 2 years \\
% P6 & 8 years & 1 year \\
% P7 & 4 years physics & 4 years \\
% P8 & 3 years industrial design & 1 year
% \end{tabular}
% \caption{An overview of the participants for the generative sessions, provided for reference.}
% \label{tab:participants}
% \end{table}

==> content/old/design-guidelines-360-VA.tex <==
\subsection{Flat 360° Video Artifacts}
\subsubsection{Full frame artifacts}
\begin{itemize}
    \item suggested projections for overall screenshots
\end{itemize}
\subsubsection{Perspective artifacts}
\begin{enumerate}
    \item Embed an overview of the 360° video (using one of the projections above)
    \item Overlay information about the orientation of the perspective (using colors and objective things)
\end{enumerate}
- this helps multi-frame screenshots (clusters, storyboards)
\subsubsection{Intra-frame Artifacts}
\begin{itemize}
    \item to create the artifacts discussed by Meijer et al, use the overview methods discussed above along with meta-frame annotations
\end{itemize}
\subsection{Spatial 360° Video Artifacts}
Inspired by the rich spatial nature of 360° video we create a number of ``spatial'' 360° video artifacts that transform from the flat-ness of a frame of video.
\subsubsection{Pseudo spheres to understand spatial relations}
\begin{itemize}
    \item understanding and aligning on spatial relations for insights is important (see intra-frame annotations)
    \item by leveraging simplified projections (full frame artifacts) it is possible to transform 360° video frames to simple 3D objects for discussion and alignment
    \item supports understanding of differences with multiple videos (by showing context quickly)
\end{itemize}

\subsubsection{artifacts for spatial-temporal insights}
\begin{itemize}
    \item pop up book style creations enable intra-inter-frame artifacts that give insight into spatial relation
    \item dollhouse makes it easier to map out how ¿different? users use a space over time
    \item creating a screenshot map keeps rich 360° context in discussion of spatial interactions (map with cylinders)
\end{itemize}






==> content/old/expand/method.tex <==
We recruited six pairs of designers using professional networks, the~\weak{summary of the experience, age, gender of the designers}. In order to familiarize the participants with the capabilities and challenges of 360° video design ethnography, each participant received one of two design tasks with the associated 360° video. These tasks were selected based on previous examples of 360° video ethnography~\cite{neubauer_experiencing_2017,porcheron_cyclists_2023}.
\begin{enumerate}
    \item You are developing a bicycle that aims to reduce traffic accidents and makes the cyclist feel more safe in the city. Use the 360° video~\footnote{link to the 360° video here.} to gather insights into how the cyclist interacts with traffic and how that might be improved.
    \item You are developing robotic assistants for astronauts that support their work and aim to make their environment more enjoyable. Use the 360° video~\footnote{\url{https://www.youtube.com/watch?v=ZfFssKBiOn8}} to gather insights into the capabilities of the robot and how they might improve the context of the astronauts.
\end{enumerate}

The workshop structure was:
\begin{table}[H]
\begin{tabular}{l p{0.5\linewidth} l}
Activity: & Description: & Time: \\
Understand video artifacts & Facilitator presented an overview of when and why video artifacts are used (Section N) and the composition of video artifacts (Section N) & 5 \\
Understand 360° video & Facilitator demonstrated what 360° video is and how it can be viewed with different projections & 5 \\
Experience challenge of creating 360°VAs & Participants were each provided with a laptop with a 360° video and design task & 20 \\
Reflect on challenges of 360°VAs & Participants engaged in a semi-structured reflection of the challenges they experienced when creating, sharing, and interpreting the 360°VAs & 10 \\
Introducing the framework & Facilitator presented the initial framework for creating 360° video artifacts (Section N) & 5 \\
Redesigning 360°VA with framework & Participants recreated their VAs using the recommendations of the framework, and reshared the artifacts & 15 \\
Reflecting on the process & Participants engaged in a semi-structured reflection and critique of the framework & 20
\end{tabular}
\caption{The workshop structure used to ensure the framework for creating 360° video was comprehensive and included input from a diverse set of designers.}
\label{tab:expand-ws-structure}
\end{table}

\weak{The framework was altered based on the outcomes of this workshop (Section N) to create the penultimate version (Appendix N). This version was used in the subsequent Reflect workshop.}


==> content/old/expand/result.tex <==
here are the changes made to the framework based on the themes and artifacts from the first set of workshops 

==> content/old/framework-evaluation.tex <==
In order to understand how 

\red{here I will describe the process of selecting two case studies to use as a way to run through using tangible 360° video artifacts through a small design process.}

The two case studies will cover:
\begin{enumerate}
    \item A use case where the camera and subject move through a space (ego-centric)
    \begin{enumerate}
        \item cycling
        \item electricity installer?
    \end{enumerate}
    \item a use case where the camera is fixed and subjects move around it
    \begin{enumerate}
        \item cooking
        \item space
        \item retirement homes?
    \end{enumerate}
\end{enumerate}

Important to note:
\begin{enumerate*}
    \item use cases should involve multiple videos (of multiple contexts
    \item use cases should illicit multi-frame artifacts
\end{enumerate*}

==> content/old/methods.tex <==
In order to ensure our initial framework for creating 360° video artifacts is comprehensive and applicable we conducted two sets of design workshops:
\begin{enumerate*}
    \item a set of workshops where designers \textbf{expanded} on the initial framework, and
    \item a set of workshops where designers used and \textbf{reflected} on the final framework.
\end{enumerate*}

\subsection{Expand Workshop}
\input{content/expand/method}
\subsection{Reflect workshop}



==> content/old/old-generative-sessions.tex <==


In order to structured the framework beyond these individual artifacts, we engaged in a series of 8 generative sessions with participants including professional designers, design researchers, experts in visual perception, and physicists working on optics. During these generative sessions, participants were guided through the material that set the context for using 360° video artifacts along with the initial artifacts (Shown in Figure~\ref{fig:initial-artifact}, and provided in Appendix~\red{N}). First, the purpose of tangible video artifacts was established using a visualization of Section~\ref{bg-conv-video-artifacts}, then the benefits of 360° video and how it impacts tangible video artifacts was described. Next, participants were shown the initial artifacts described in Section~\ref{initial-framework} and engaged with the lead researcher in reflecting on the differences between the artifacts, how they would or would not be used, as well as modifying the artifacts as well as creating new ones. We used observations, comments, and direct input from participants which elicited the following concepts: 

\begin{enumerate}
    \item The different artifacts lay on a spectrum with a few possible labels, guiding the selection of artifacts based on the purpose and moment in the video design ethnography process.
    \item 360° content elicits the need for two elements: a connection between details and overview, as well as establishing spatial orientation and alignment.
    \item The framework should provide guidelines for creating conventions that support design teams with the first two concepts, rather than provide a singular prescriptive approach.
\end{enumerate}
are shown in Figure~\ref{fig:gen-session-framework}, with the design space of the different artifacts shown on the left and conventions that support connection and orientation shown on the right.
\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{content/images/generative-session/initial-framework.jpg}
    \caption{The first version of the Tangible 360° Video Artifact Framework synthesized from generative sessions. The left side showing the design space of tangible 360° ``frame'' elements. The right shows several conventions that address challenges identified during the sessions.}
    \label{fig:gen-session-framework}
\end{figure}
\subsection{The Design Space of Tangible 360° Video Artifacts}
During the sessions, participants described many ways that the different 360° video artifacts related to each other; specifically drawing the relation between the flat and volumetric boundary objects as ``focused'' -- ``immersive'', ``specific'' -- ``exploratory'', ``seeing'' -- ``feeling'', and ``a very human view'' -- ``a god like perspective''. Crucially, participants related these dimensions to different goals at different stages of video design ethnography: starting with an immersive overview using the volumetric objects, transitioning to flat artifacts to focus on specific details, and then going back to the overview again. Therefore we present this gradient as one of the dimensions of the design space of tangible 360° video artifacts, and leave the selection process up to the needs of a specific moment in the design process.


\subsection{Connection and Orientation}
Beyond acting as a 360° ``frame'' -- i.e., a tangible representation of designers' insights -- participants noted that 360° content requires artifacts to support two elements:
\begin{enumerate*}
    \item \textbf{connecting} specific details that inform analysis to where they exist in the 360° frame, and
    \item joint \textbf{orientation} of events, actors, and the spatial relations between them in the 360° frame.
\end{enumerate*}
These two actions further demonstrate the difference between the flat and volumetric artifacts -- flat artifacts show the details but need a connection to the overall context (e.g., by including a mini-map) were as volumetric artifacts show the whole but need a connection to specific details.

\subsection{Conventions}
Participants differed widely in their preferences for different artifacts, but were unanimous that the choice of artifact and modifications to it were highly dependent on the goal of the artifact, stage of the design process, preferences of the designers, and other factors. This aligns with the concept of that the artifacts used to communicate ideas vary and evolve throughout the design process~\cite{dalsgaard_emergent_2014}.

This discussion elicited the concept of using ``conventions'' -- commonly understood methods to select, create, and modify the video artifacts within a design team -- instead of prescribing the use of the artifacts. Therefor the framework aims to show what conventions should be established, and provide examples of these conventions. Figure~\ref{fig:gen-session-framework} lists a number of these conventions which are explained in Table~\ref{tab:conventions}.

\begin{table}[]
\begin{tabular}{m{2cm}|m{2cm}|m{2cm}|p{6cm}}
Artifact type & Goal & Convention & Description \\ \hline
Flat & detail-context & mini-map & Including the entire 360° frame in a mini-map, flat artifacts can include the full context and their place in it. \\
Flat & orientation & graticules & Graticules provide information about the perspective and location of a flat artifact in the larger 360° context. \\
Flat & orientation & set perspectives & Using a limited set of perspective when creating flat artifacts reduces complexity and means designers can develop understanding of a few distorted views. \\
All & detail-context & links & Flat and volumetric artifacts can work together by linking detailed flat artifacts to volumetric ones physically or via meta-frame annotations. \\
All & orientation & semiotics & Using symbols such as naming locations, color coding areas of the frame, etc. to embed orientation information into the artifact. \\
Volumetric & detail-context & desaturation & Applying post-processing to draw attention to specific details in the overall context while maintaining the entire visual field. \\
Volumetric & orientation & facet alignment & Aligning the facets of the artifact with elements of the context (e.g., streets, the subject of the video, magnetic north) supports orientation and alignment of multiple artifacts.
\end{tabular}
\caption{Examples of types of conventions elicited during the generative sessions.}
\label{tab:conventions}
\end{table}

==> content/old/old-introduction.tex <==
Designers use video as material to gain insight into the context and actions of potential users of their design~\cite{nova_beyond_2014,ylirisku_designing_2007}. Video enables designers to observe in real-time interactions that might otherwise be difficult or dangerous to observe in person~\cite{paay_connecting_2015,lamas_analyzing_2019,nielsen_using_2023,komkaite_underneath_2019}, while also being able to replay the video many times in the future~\cite{ylirisku_designing_2007}. Thus, video enables designers to get a rich, dynamic window into the context they are designing for. The process by which they engage with video is referred to as Video Design Ethnography (VDE), and involves designers viewing, annotating, and collaborative analyzing video to extract insights, which are the output of VDE shared with other stakeholders~\cite{nova_beyond_2014,ylirisku_designing_2007}.

The increasing ubiquity of easy to use consumer 360° video cameras~\cite{jokela_how_2019} has lead to the increased use of 360° video for ethnographic studies~\cite{gomez_cruz_immersive_2017,vatanen_experiences_2022}, since 360° video captures the entirety of the visual context, and thus no actions take place out of frame~\cite{tojo_how_2021} (as seen in Figure~\ref{fig:360-why}). Additionally, 360° video enables designers to immerse themselves in the world of the user and take the perspective of different actors in an interaction~\cite{tojo_how_2021,vatanen_experiences_2022,kramer_innovating_2022}. 

\begin{figure*}[]
    \centering
    \subfloat[A frame of conventional video.]{\label{fig:conventional-video}\includegraphics[width=0.45\textwidth]{content/images/demonstrating 360/just-pers.png}\Description{A few cars are on a street in Paris.}}
    \qquad
    \subfloat[The full 360° view of the same frame.]{\label{fig:360-full-frame}\includegraphics[width=0.45\textwidth]{content/images/demonstrating 360/360-frame-info.jpg}\Description{A distorted picture of someone biking around the street, much more visual information is shown.}}
    \caption{The difference in visual information of a frame when using conventional video and 360° video for an exemplar use case of studying cycling behavior, similar to~\citet{porcheron_cyclists_2023}. The 360° video contains a lot of information and interactions that is ``out of frame'' in the conventional video, however the 360° frame is heavily distorted.}
    \label{fig:360-why}
\end{figure*}

However, the fact that 360° content is spherical makes sharing 360° content challenging~\cite{jokela_how_2019,tojo_how_2021}, a viewer can see either a subset of the video (Figure~\ref{fig:conventional-video}) or a distorted view of the entire 360° video (Figure~\ref{fig:360-full-frame}). This means that, to share an insight from 360° video, designers need to either use an image with distortion (the full frame), crop the image so it is not distorted (removing all the contextual information of 360° video), or partially crop the image (resulting in both distortion \textbf{and} removing contextual information). Therefor, collaboratively viewing or sharing moments from 360° video is a largely unaddressed challenge~\cite{jokela_how_2019,tojo_how_2021}.

This makes the adoption of 360° video for VDE challenging -- collaborative sense-making and analysis requires designers to share their insights from videos quickly and easily~\cite[p. 126]{ylirisku_designing_2007} to identify common elements or new directions for re-evaluating the video. Recently,~\weak{Meijer et al.} explored how 360° video impacts these collaborative video workshops, noting that designers struggled using ``perspective screenshots''(such as Figure~\ref{fig:conventional-video}) to communicate their insights, especially insights that took advantage of the 360° nature of the video. In the terms of VDE, these screenshots are used as ``video artifacts'', tangible elements taken from video to share insight(s) between designers during sense-making, or to other stakeholders as the output of a design research process~\cite{ylirisku_designing_2007,nova_beyond_2014}.  

Therefor, we set out to create Tangible 360° Video Artifacts -- that is, video artifacts based on 360° content, that fit into the tangible and collaborative processes of Video Design Ethnography.
We start by describing two classes --flat and sphere-ish-- of tangible 360° ``screenshots'' (Section~\ref{tool}). We use these initial artifacts to engage with experts in generative sessions to reflect on the useful qualities of artifacts (Section~\ref{generative-sessions}), which elicited the importance of \textit{orientation} and \textit{linking} as functions specific to \textit{360°} artifacts -  as well as some early meta and multi frame artifacts. Finally, we discuss the implications of Tangible 360° Video Artifacts, limitations of this early work, and future steps to expand on these artifacts as well as further understand their impact on collaborative design work.

To summarize, this paper's key contributions include:
\begin{itemize}
    \item Introducing and motivating the concept of Tangible 360° Video Artifacts for VDE.
    \item An open source tool to quickly create two distinct classes of Tangible 360° Video Artifacts (and the design decision behind these artifacts).
    \item A thematic analysis of the (envisioned) use and extension of the Tangible 360° Video Artifacts created by our tool.
\end{itemize}

==> content/old/reflect/method.tex <==
\weak{here is the method of the second workshop}

==> content/old/reflect/result.tex <==
\weak{here are the resulting findings and themes that show how the framework can be used}

==> content/old/related-work.tex <==
\subsection{Video Design Ethnography}
Design ethnography denotes how designers and user researchers study (potential) users in order to gain insights that are used to develop new products and services~\cite{salvador_design_1999}. 
While many forms of information that can be used in design ethnography,~\citet{ylirisku_designing_2007} eloquently notes that ``video is the medium that conveys most of the detailed richness of a real setting, as compared with text, photos and audio recordings''. 
This richness stems from video's multi-modal (combining visuals and sound) and temporal (the images and sound change over time) affordances.

\begin{itemize}
    \item This rich nature means there are many techniques to use video in design ethnography; with different forms of video such as in-situ recordings, video diaries, and interviews~\cite{nova_beyond_2014,ylirisku_designing_2007}, and a multitude of methods to analyze video~\cite{vannini_routledge_2020}.
    \item \citet{nova_beyond_2014} provide a generalized framework for the process of design ethnography, defined by six stages:
    \begin{enumerate*}
        \item brief
        \item preparation
        \item research design
        \item field research
        \item analysis
        \item design intervention
    \end{enumerate*}
    \item While each of these stages are important to design ethnography, the bridge between the final two stages analysis and design intervention requires designers to overcome ``the challenge of conveying their understanding''~\cite{ylirisku_designing_2007} to other stakeholders.
    \item To this end, designers create ``video artifacts'' - artifacts created using elements from the videos that are used to share and align on information during the analysis phase.
\end{itemize}

% \subsection{Video Artifacts as Boundary Objects}

% We used the term ``video artifacts'' to refer to boundary objects used to communicate and align the insights generated from video design ethnography between designers and other stakeholders (other designers, engineers, clients, etc.)~\cite{ylirisku_designing_2007,nova_beyond_2014}. 
% Examples of video artifacts include storyboards, video collages, and video mangas. A more complete overview is provided in Section~\ref{bg-conv-video-artifacts}.

% It is important to note that boundary objects have distinct qualities; they are a communication tool (they are made with the intent of sharing information by one group to others), they are often auxiliary artifacts (not the primary output of the design process), and emergent (the type and number of boundary objects are influx)~\cite{dalsgaard_emergent_2014}.
% This reinforces the idea that video artifacts are meant to communicate the insights of the designers, are auxiliary to the design intervention (i.e. they support the understanding but are not the product), and take many forms depending on the needs of the design process. 

% \subsubsection{(Static) Video Artifacts}
% One important distinction in the scope of this work is the difference between ``video, video artifacts'' (i.e., artifacts that \textit{are} videos) and ``static video artifacts'' (i.e., artifacts that \textit{use} elements of the video, but are not videos themselves). 
% This is the difference between the Video Collages described by~\citet{ylirisku_designing_2007}, where designers edit clips together to illustrate a theme found in analysis, with the more general collage described by~\citet{nova_beyond_2014} where designers select still frames to illustrate a theme instead.

% There are two pragmatic reasons for focusing on static video artifacts: they are easier to share, and they are more restricted.
% First, sharing static artifacts is simpler because they do not require as much time to view as videos, are easier to include in reports, and can be printed and made tangible, which is desired in workshops~\cite{nova_beyond_2014}. 
% Second, static video artifacts are more restricted, they remove the two affordances of video (time and audio), which makes transforming videos into static artifacts a non-trival process~\cite{uchihashi_video_1999}.

\subsection{Benefits of 360° Video for Design Ethnography}
\begin{itemize}
    \item 360° video has a lot of power to make insights richer
    \item 360° video does this because it is more immersive and has more context by adding the affordance for the designer to change the perspective
    \item some examples of why 360° video is cool
    \item 
    \item previous work has highlighted the ease at which designers can integrate 360° video into early stages of the design ethnography cycle (brief, preparation, research design, and field research), however~\weak{Meijer et al.} describe how 360° imagery is more challenging for designers to share in collaborative workshops.
\end{itemize}


==> content/old/toolkit.tex <==
In order to enable the creation of the example artifacts in Section~\ref{case-study} and support the use of Tangible 360° Video Artifacts by practitioners, we developed the Tangible 360° Video Artifact Toolkit -  a web based toolkit with three main components:
\begin{enumerate}
    \item a set of guidelines for selecting between the classes of artifact discussed in Section~\ref{initial-framework},
    \item a tool to create the Flat artifacts from 360° frames, and
    \item a tool to create cut and fold patterns to create Sphere-ish artifacts from 360° frames.
\end{enumerate}

Below we briefly describe the tools which are available on~\url{v1.360artifact.com} and the source code and an explanation of the underlying technology is available on~\url{v1.360artifact.com/source}. Figure~\red{add figure} provides examples of the two tools creating artifacts using the same image, and the guidelines are provided below.

\subsection{The Guidelines}
The guidelines are based on the differences in impression (\ref{result:difference-in-impression}) and use (\ref{result:difference-in-use}) of the classes of artifact noted by participants during the generative sessions and reads as follows:

In order to support your use of 360° video in collaborative design workshops, we provide tools to create two different types of artifacts: flat (Figure [A])and sphere-ish (Figure [B]). 
The flat artifacts are 2 dimensional and show a specific detail or set of details in a larger 360° frame. They provide an \textbf{analytical} and \textbf{human-level insight} and are thus useful for detailed analysis of specific moments or themes that were found to be relevant.
The sphere-ish artifacts are 3 dimensional and provide a \textbf{more-than-human} or \textbf{atmospheric} overview of the entire 360° video. This means that sphere-ish artifacts are useful for understanding the overall environment of a video, understanding spiritual relations in the entire frame, or as a singular token of a moment.
These artifacts present two initial directions for using 360° material in collaborative design workshops and you will undoubtedly encounter novel uses, benefits, or challenges -- or even develop entirely new artifacts -- as this is an ongoing research project into the use of 360° video and the tools and artifacts to support it, please feel free to reach out to \url{contact@360artifact.com} to share your insights, artifacts, or otherwise engage with the researchers.


% \subsection{Flat Artifact Tool}
% The flat artifact tool simply allows the user to upload a 360° image, select an area of interest, and select if they want to implement graticules and/or a minimap. The tool then exports the resulting flat video artifact.

% \subsection{Sphere-ish Artifact Tool}
% The sphere-ish artifact tool simply allows the user to upload a 360° image, adjust the ``rotation'' of the image so the resulting facets of the artifact align with directions (see~\ref{result:orientation}), and then select between several cut and fold patterns that were pre-generated using Blender~\footnote{A popular open source 3D modeling tool,~\url{https://www.blender.org/}} and the Paper Model extension~\footnote{That creates cut and fold patterns for 3D models,~\url{https://docs.blender.org/manual/en/latest/addons/import_export/paper_model.html}}.
